NaijaHate: Evaluating Hate Speech Detection on Nigerian Twitter Using Representative Data

To address the global issue of online hate, hate speech detection (HSD) systems are typically developed on datasets from the United States, thereby failing to generalize to English dialects from the Majority World. Furthermore, HSD models are often evaluated on non-representative samples, raising concerns about overestimating model performance in real-world settings. In this work, we introduce NaijaHate, the first dataset annotated for HSD which contains a representative sample of Nigerian tweets. We demonstrate that HSD evaluated on biased datasets traditionally used in the literature consistently overestimates real-world performance by at least two-fold. We then propose NaijaXLM-T, a pretrained model tailored to the Nigerian Twitter context, and establish the key role played by domain-adaptive pretraining and finetuning in maximizing HSD performance. Finally, owing to the modest performance of HSD systems in real-world conditions, we find that content moderators would need to review about ten thousand Nigerian tweets flagged as hateful daily to moderate 60% of all hateful content, highlighting the challenges of moderating hate speech at scale as social media usage continues to grow globally. Taken together, these results pave the way towards robust HSD systems and a better protection of social media users from hateful content in low-resource settings.

==> data_old.tex <==
\subsection{Data}\label{sec:data}

\paragraph{Hate words and targeted communities}\label{hate_target_lists}
\Karim{Moved this chunk below from related work}
Previous studies on online hate speech have defined hate speech categories (e.g., ‘hateful’, ‘offensive’ and ‘neutral’) based on different strengths of abuse classification \cite{davidsonetal2017}, a strategy that best aligns with current content moderation policy.
Defining hate speech can be a contentious task, labeling decisions are inherently subjective when there is a lack of consensus on whether a sentence is hateful. Key to the detection of hate speech is the creation of high-quality annotated data, necessitating annotation guidelines that are clear and comprehensive. 

\Karim{Introduce why we need these sets : random sampling would yield few positives, so we need to stratify the data. This is why we collect hate words. Additionally, we stratify also for targeted communities as hate speech by definition needs to target communities.}
\Karim{Define "hate" here.}
\Karim{Restructure : this is only for hate speech}
% To this end, we next present the annotation strategy suited for active learning used to train our models. 
% We first draw a stratified sample of tweets that can then be annotated and used for supervised learning\karim{what task ?}.
% \Karim{It is unclear what is stratified, the paragraph title mentions both hate detection and target detection. We could be more specific ?} To this end, w
We define a list of seed words that often appear in hate speech in the Nigerian context. 
%Specifically, our list contains 3 categories of words: Nigerian-specific derogatory words, names of communities often targeted by hate speech in Nigeria and words combining a derogatory word and a community name (e.g. ``fulanimal''). 

We first build a list of 84 Nigeria-specific hate terms. To do so, we rely on lexicons from past work on the topic \cite{udanor2019combating, farinde2020socio}, Nigerian online dictionaries as well as local knowledge from Nigerian colleagues. 
%The final list contains 27 Yoruba words, 26 English words, 13 Hausa words, 9 Pidgin words and 7 Igbo words. %\Manu{need to double check the numbers}
% \footnote{Specifically, those experts are consultants who are native speakers of the different dialects.} 
% words collected from the urban dictionary\footnote{\url{https://www.urbandictionary.com/}}\karim{is this the website?}

Second, we define a list of names of communities that are often targeted by hate speech in Nigeria, again relying on local knowledge from Nigerian colleagues.
% to build this list and we restrict the initial list of community names to the names in this that are most frequently mentioned on Nigerian Twitter. 
This approach yields 12 communities, including 5 ethnic groups (Yoruba, Igbo, Hausa, Fulani, Herdsmen\footnote{Herdsmen are not a ethnic group per se but this term refers exclusively to Fulani herdsmen in the Nigerian context, hence the categorization as an ethnic group.}), 2 religious groups (Christians and Muslims), 3 regional groups (Northern, Southern, Eastern) and 2 groups on gender identity and sexual orientation (Women and LGBTQ+).  For each of these groups, we list the different denominations of each group as well as their plural form and combine it in regular expressions, referred to thereafter as \textit{community regular expressions}. Finally, we also identify 5 words combining a community name with a derogatory word (e.g. ``fulanimal'') that we coin \textit{combined word} thereafter. 

We provide the full list of hate, community and combined words and the community regular expressions in Section \ref{appendix:word_lists}. \Manu{To do: add frequency, regex}
% \Karim{This portion is a bit long and contains some details that could go in the appendix. Would make it half a column}

% On the other, we create a dictionary of words associated with selected communities for target inference, in order to generate a community set relying on keyword and regular expressions matching, to cover the various ways these communities are talked about. In doing so, we chose to focus on the 12 most frequently mentioned communities, as this subset covers a large share of the Nigerian population. \karim{We need figures to support this claim: do we have stats?}
% We are aware that our matching doesn't capture all tweets mentioning a given community. However, these community sets are only the starting point for our active learning approach, detailed subsequently. 

% \Karim{As far as I understand we also annotated tweets in a random sample, we need to mention this and eventually give names to the sets in bold e.g. "community set" for AL training and "random test set" for evaluation purposes} 
% Additionally, we manually annotated a random sample for evaluation, independently from the automatic matching for community sets.

\paragraph{Twitter dataset}
Our Twitter dataset was collected from the Twitter API. It contains the timelines of 2 million Twitter users with an inferred profile location in Nigeria. In total, this amounts to about 1 billion tweets posted between January 2007 and December 2021. The language of the tweets is mostly English (76\%) according to the Twitter language detector though we observe that an important share of these can be categorized as Nigerian Pidgin English. We provide more details on the tweet collection in Section \ref{appendix:tweet_collection} of the Appendix.
% Starting with a seed list of users with an inferred profile location in Nigeria and who posted at least one tweet in the Twitter Decahose, a 10\% random sample of all tweets ever posted, we employed a snowball sampling strategy to curate a comprehensive sample of 2 million Nigerian Twitter users. This process resulted in a dataset of approximately 1 billion tweets. Recent estimates from the fact-check organization Africa Check\footnote{ttps://africacheck.org/fact-checks/reports/forty-million-twitter-users-nigeria-how-pollsters-flawed-figure-became-fact} suggest that Nigeria has about 3 million Twitter users, which indicates that our dataset provides an excellent coverage of the Nigerian Twitter population. \Manu{say something about the language of the tweets}

We consider two separate settings to develop and evaluate our hate speech detection model. The first one is the subset of tweets where at least one community often subject to hate speech is mentioned, referred to as the \textit{community set} thereafter. In this set, the prevalence of hate speech is presumably higher, reducing the class imbalance and simplifying its detection. We build this set by selecting the subset of tweets that match with at least one of the community regular expressions defined earlier, totaling 42 million tweets. We then randomly split this community set into two equally-sized sets $C_s$ and $C_e$ that we use respectively for sampling and evaluation. Second, we aim to build a detection model that is robust to real-world conditions of extreme class imbalance. For this purpose, we draw a random sample of 200 million tweets out of the full Twitter dataset. As previously, we then split it randomly into two equally sized sets $F_s$ and $F_e$ that we use respectively for sampling and evaluation.

\input{tables/target_hate_examples}

\paragraph{Data annotation}
% \Karim{Instead of having a "hate words and targeted communities" AND "Data annotation" paragraph, I would have a "Hate speech" paragraph and a "Targeted community" paragraph, where both the auxiliary data (words, etc) and annotation processes are described. I'd also present the stratified sample in the first one, and split evaluation between each}
% \Manu{The stratification is based on hate words + community words so it concerns both and cannot only appear in an independent hate speech paragraph}
% The subsequent tweet annotation of tweets is two-fold. 

First, our labeling process seeks to identify three mutually exclusive speech categories that a tweet may belong to: hateful, offensive or neutral. Following past literature \cite{rottger-etal-2021-hatecheck}, we define hatefulness as an attack on an individual or a group based on the perceived possession of a protected characteristic such as a certain gender or race. 

Second, for tweets characterized as hateful, annotators are asked to define the communities targeted by the tweet among our list of communities defined in the previous subsection. We provide examples of tweets targeting each of our communities of interest in Table \ref{tab:target_hate_examples}.
%\manu{We don't have a precise question that we asked annotators so no precise questions in the annotation guidelines in the Appendix for now}
% For the annotation process, we choose a prescriptive approach \cite{rottger2021two}, providing a single definition of hate in our guidelines and asking the annotators to follow these guidelines during labeling. Such guidelines are described in greater detail in Section \ref{appendix:labeling_guidelines} of the Appendix. 

The data is annotated by a team of 4 Nigerian colleagues. We provide further details on data annotation in Section \ref{appendix:annotation}.
% While we chose a prescriptive approach \cite{rottger2021two} to allow for policy relevance in light of content moderation, we account for cultural differences \cite{maronikolakis2022-listening} by engaging a diversity of annotators who were guided by a field coordinator with regional expertise. \Fixme{[More details on this pool of annotators]}

% \Todo{Include definition, references for guidelines. All tweets labeled at least twice and three times in case of disagreement (in case of disagreement with three labels, drop; if unsure label + ibrahims label, ibrahims has priority).} 

% \manu{Potentially make a table with examples of hate against each community}

% \paragraph{Sampling and evaluation random samples}

% While most hate speech classifiers are evaluated on random samples of curated datasets where the class imbalance is limited, we aim to evaluate our classifier in real-world settings of extreme imbalance. Specifically, we aim to evaluate our classifier (i) in the subset of all tweets containing at least one community name on the one hand, and (ii) on all tweets on the other hand.

% First, using the community regular expressions defined earlier and detailed in Section \ref{appendix:word_lists}, we select the subset of tweets that match with at least one community regular expression, totaling 42 million tweets and referred to as the \textit{community set} thereafter. We then randomly split this community set into two equally-sized sets $C_s$ and $C_e$ that we use respectively for sampling and evaluation. 

% Second, we draw a random sample of 200 million tweets out of the full Twitter dataset. As previously, we then split it randomly into two equally sized sets $F_s$ and $F_e$ that we use respectively for sampling and evaluation.
% \Fixme{Say a word on the fact that most classifiers are evaluated on curated/small datasets, not clear how they perform in real-settings of extreme imbalance}



% \Karim{Would put both "Data annotation" and "Initialization sample" in the appendix, or move to the previous section}
% \Manu{@Karim: with the new structure, I think it's important to keep them }

\paragraph{Initialization sample}
\Karim{Changer ça en : we annotate a sample for HSD et bouger la partie "initialization sample" dans "Active learning"}
\Karim{Sert à tester toutes les méthodes, dataset labellé, puis sert d'initialization sample.}
As previously stated\manu{this must be stated earlier in intro and/or related work}, the extreme imbalance in our classification task makes random sampling ineffective and prohibitively expensive. With the aim to build high-performing classifiers at a reasonable cost, we build and annotate a stratified sample of tweets from the community sampling set $C_s$. We use three different sampling strategies to build this stratified sample. First, for each possible combination of community name and hate word, we sample up to 4 tweets that both contain the respective hate word and match with the respective community regular expression. Second, for each combined word W, we randomly sample 50 tweets containing W. Finally, for each community, we draw 50 random tweets matching with the community regular expression, in order to avoid having a classifier that associates the community name with hate speech.

This yields a stratified sample of 1,607 tweets annotated as either hateful, offensive or neutral, including 528 hateful tweets with annotated targets. We provide more information on the sampling procedure and on the initial stratified sample in Section \ref{appendix:initial_sample}.

==> old_results.tex <==
\subsection{Hate Speech Detection}

\paragraph{Stratified sampling}
We evaluate our models for hate speech detection on the stratified sample described in \cref{sec:hsd_methods}, both for the 3-class detection task described earlier, and a binarized version where offensive and neutral tweets are considered collapsed into the same class. We report the results in Table\ref{tab:hate_speech_evaluation_stratified}. 

Our main finding is that Supervised Learning, based on the Conversational BERT architecture,
% \karim{give this a name like ConvBERT and use it here and in table}\manu{problem is ConvBERT is another model: \url{https://huggingface.co/docs/transformers/model_doc/convbert}}, 
performs best overall and outperforms the off-the-shelf methods on both tasks. Among off-the-shelf methods, $GPT_{3.5}^{ZSL}$ and $GPT_{3.5}^{FSL}$ outperform the Perspective API in terms of F1 score on the binary classification task, despite not being tailored for toxicity detection as Perspective is. We also find that few-shot learning counterintuitively appears to worsen the performance on both classification tasks compared to a zero-shot setting. %A possibility could be that the tested models overfit the few examples they are given in this setting, failing to generalize to unseen ones. 
We further note that both off-the-shelf methods exhibit a decent performance well above the rule-based baselines in the Nigerian low-resource context. This means that recent models mostly trained on US English data make it possible to reach acceptable though not excellent performance in other low-resource English dialects, despite requiring zero annotation efforts. Finally, we note that the performance of our models on the binary task strongly exceeds the one on the 3-class version, which is largely explained by the rather poor performance for the offensive class as observed in the related confusion matrix (Figure \ref{fig:confusion_matrix_3_class_hsd} in the Appendix). This difficulty to disentangle offensive and hateful speech can partly originate from the similarities between offensive and hate speech, such as the common use of slurs.

Despite a dominance of Supervised Learning over other approaches, its performance at HSD, especially in the 3-class setting, is not satisfactory. Next, we explore whether AL, and specifically Certainty Sampling, can further improve the performance of Supervised Learning on our 3-class detection task at a low labeling cost and under real-world settings of extreme imbalance.

% \Manu{support this final claim with confusion matrices in Appendix (still need to produce them)}


% \Todo{Off-the-shelf models have satisfactory performance in a low-resource context (probably because language basis remains English for which both tools are most performant). GPT3.5 outperforms Perspective API which is impressive because the latter is specialized for hate speech detection while the former is not ( FSL not improving results}

% \Manu{[unfeasible to evaluate in the wild as in previous part because of API costs for ChatGPT and rate limits for Perspective API]}


\input{tables/evaluation_hate_speech_detection_stratified}

% \manu{talk about how the performance of SL on the stratified sample is not great, especially for 3-class; look at AL to further improve the performance in the wild}
% \paragraph{Active learning}



% \paragraph{Impact of sampling on target inference}
% \Todo{A cost of the improved performance at HSD is that the imbalance in the target inference dataset grows. As observed in Figure \ref{fig:AL_results_share_community_per_target}, AL samples disproportionately hateful tweets targeting some communities compared to others (e.g. women, fulani). A possibility is that hate against these groups is more common, or also that it is more ambiguous and the model struggles to detect this type of hate (e.g. lots of tweets of victims from Fulani herdsmen denouncing the killings but not hateful towards Fulanis = ambiguous).}




% \subsection{Comparison of Supervised Learning with existing off-the-self baselines}

% \paragraph{Hate speech detection}

% Comparison between BERT-based Supervised Learning and off-the-shelf methods (ChatGPT ZSL and Perspective)

% \Manu{[unfeasible to evaluate in the wild as in previous part because of API costs for ChatGPT and rate limits for Perspective API]}
% \Manu{We can potentially add ChatGPT few-shot if we have time}

% \input{tables/evaluation_hate_speech_detection}

\subsection{Target inference}

Next, we conduct TI on a sample of top-scored tweets resulting from the inference on a large random sample of tweets of our best performing Supervised Learning model, namely Conversational BERT at iteration 24 of Certainty Sampling. We report the accuracy and F1-scores in Table \ref{tab:target_inference_results} and the target-level F1 scores in Figure \ref{fig:performance_target_level_ti} in the Appendix.  

Our main finding is that Supervised Learning largely outperforms both zero and few-shot learning on the one hand and Regex matching on the other hand in terms of accuracy and macro-F1 score. This finding also holds on the stratified sample (see Table \ref{tab:target_inference_results_stratified} in the Appendix). In line with HSD, we find that FSL slightly deteriorates the classification performance, also possibly due to over-fitting. When investigating the errors of the different models, regex matching is sensitive to variations in the spelling of community names (e.g. notherner), which calls for an extension of the existing community regular expressions. It also misinterprets self-references as hate towards the author's group (e.g. "I'm Yoruba and I hate Hausas"). On the other hand, $GPT_{3.5}$, despite being prompted to only list targets belonging to our 12 communities of interest, tends to include every subject in the tweet that are potentially targeted by hate, such as usernames. Some groups identified by the model are correct but we observe that the model lacks the domain knowledge to assign some predictions into the group they belong to. For instance, ``Arewa'', which is the Hausa word for ``North'', should be but is not associated to the ``Northerners'' target group. 

At the target level, we find that the performance gap between the best and least performing target classes is smaller for Supervised Learning compared to $GPT_{3.5}$ and regex matching indicating a better fairness of Supervised Learning. Igbos, followed by Hausas and Muslims are the classes with the worst individual F1 score while targets such as Christians, Southerner and Herdsmen have a perfect F1 score of 1 (Figure \ref{fig:performance_target_level_ti} in the Appendix). These differences cannot be fully explained by class imbalance as the worst performing classes are more represented in the training set than some of the best performing classes such as Christians and Southerners (Figure \ref{fig:target_share_train_test} in the Appendix). When investigating the misclassifications, we find that the targets with a lower performance are characterized by a higher number of denominations for the same community (e.g Aboki for Hausas), as opposed to the best performing targets which are consistently characterized by one term (e.g. Christians), making it harder for the model to pinpoint the targeted community.
% \Fixme{ChatGPT sometimes finding the right target but not grouping it into the right group (even if trivial: "the north" and "Northerners"), sensitive to typos (e.g. Nothern)}
\input{tables/evaluation_target_inference_eval_tweets}
% \Fixme{2 main phases, AL on the community set and AL on the full set}

==> section3_old.tex <==
\section{Experimental Setup}

% \Karim{Three subparts : (1) Data (2) Models and Baselines (3) Tasks}
% We develop two tools: (1) hate speech classifier and (2) target inference model 

% \Manu{intro sentence to explain the plan for this section? e.g. "our goal is XXX; after describing XX, we do XXX"}
% \Manu{I think that the sentence you wrote @Karim would work well here: "Our goal is to detect hate speech in Nigerian tweets along with the target of hate, with low labeling efforts. "}
\subsection{Tasks}
Our detection pipeline consists of a two-step process: (1) HSD and (2) TI on the predicted hateful tweets from the first step.

% First, our labeling process seeks to identify three mutually exclusive speech categories that a tweet may belong to: hateful, offensive or neutral. 
%\manu{We don't have a precise question that we asked annotators so no precise questions in the annotation guidelines in the Appendix for now}
% For the annotation process, we choose a prescriptive approach \cite{rottger2021two}, providing a single definition of hate in our guidelines and asking the annotators to follow these guidelines during labeling. Such guidelines are described in greater detail in Section \ref{appendix:labeling_guidelines} of the Appendix. 
We frame HSD as a multi-class classification problem where each tweet is classified into one of three mutually exclusive categories (‘hateful’, ‘offensive’ or ‘neutral’). Following past literature \cite{rottger-etal-2021-hatecheck}, we define hate speech as an attack on an individual or a group based on the perceived possession of a protected characteristic such as a certain gender or race. 
% \footnote{For more information on how these labels were assigned, please refer to \cref{app:annotation-guidelines}} 

%Second, for tweets characterized as hateful, annotators are asked to define the communities targeted by the tweet among our list of communities defined in the previous subsection. 
Subsequently, we aim to determine the target of each predicted hateful tweet by the previous classifier. We frame TI as a multi-label classification problem where the possible targets are 12 communities we identified to be often targeted by hate speech in Nigeria and that appear frequently enough on Nigerian Twitter. These communities include 5 ethnic groups (Yoruba, Igbo, Hausa, Fulani, Herdsmen\footnote{Herdsmen are not a ethnic group per se but this term refers exclusively to Fulani herdsmen in the Nigerian context, hence the categorization as an ethnic group.}), 2 religious groups (Christians and Muslims), 3 regional groups (Northern, Southern, Eastern) and 2 groups on gender identity and sexual orientation (Women and LGBTQ+). We provide examples of tweets targeting each of the selected communities in Table \ref{tab:target_hate_examples} and more information on the community selection process in Section \ref{appendix:word_lists}. 

% For both classification problems, we consider both supervised learning and off-the-shelf models.
% \Karim{Would put the info that 4 nigerian colleagues annotated the data in the appendix, and remove ref to appendix below.}
% The data is annotated by a team of 4 Nigerian colleagues. We provide further details on data annotation in Section \ref{appendix:annotation}.

\input{tables/target_hate_examples}

\subsection{Data}\label{sec:data}
\paragraph{Twitter data collection}
Our Twitter dataset was collected from the Twitter API. It contains the timelines of 2 million Twitter users with an inferred profile location in Nigeria. 
% In total, this amounts to about 1 billion tweets posted between January 2007 and December 2021. 
The tweets are mostly written in English (76\%)\manu{number needs to be corrected} according to Twitter's default language detector, though we observe that an important share of these can be categorized as Nigerian Pidgin English. We provide more details on the tweet collection in Section \ref{appendix:tweet_collection}.
% Starting with a seed list of users with an inferred profile location in Nigeria and who posted at least one tweet in the Twitter Decahose, a 10\% random sample of all tweets ever posted, we employed a snowball sampling strategy to curate a comprehensive sample of 2 million Nigerian Twitter users. This process resulted in a dataset of approximately 1 billion tweets. Recent estimates from the fact-check organization Africa Check\footnote{ttps://africacheck.org/fact-checks/reports/forty-million-twitter-users-nigeria-how-pollsters-flawed-figure-became-fact} suggest that Nigeria has about 3 million Twitter users, which indicates that our dataset provides an excellent coverage of the Nigerian Twitter population. \Manu{say something about the language of the tweets}

% \Karim{Unclear whether this below should stay here}
% We consider two separate settings to develop and evaluate our hate speech detection model. 
\paragraph{Data annotation}
We recruited a team of 4 Nigerian annotators through word-of-mouth, representing each major Nigerian ethnic group and gender group equally. Each annotator was tasked to annotate tweets as either hateful, offensive or neutral, and if hateful, to select the target(s) of the attack among the 12 previously mentioned communities. Annotators were compensated at an hourly rate of 12\$, well above the Nigerian minimum wage. We further describe the annotation process and describe the annotation guidelines in Section \ref{appendix:annotation}.

\paragraph{Hate speech detection dataset}
\label{hate_target_lists}

As previously stated, the extreme imbalance in our classification task makes random sampling ineffective and prohibitively expensive. With the aim to build a high-performing classifier at a reasonable cost, we use stratification to oversample hateful tweets which target our communities of interest. For this purpose, we build a list of 89 Nigeria-specific hate terms (see full list in Section \ref{appendix:word_lists}), relying on lexicons from past work \cite{ferroggiaro2018social, udanor2019combating, farinde2020socio} and Nigerian online dictionaries. We then use three different sampling strategies using the hate words and the names of the 12 previously mentioned communities to build this stratified sample. First, for each possible combination of community name and hate word, we sample up to 4 tweets that both contain the respective hate word and match with the respective community regular expression. Second, for each word W combining a hate word and a community name (e.g. ``fulanimal''), we randomly sample 50 tweets containing W. Finally, for each community, we draw 50 random tweets containing at least one community name, in order to avoid having a classifier that associates the community name with hate speech.

This yields a stratified sample of 1,607 tweets annotated as either hateful, offensive or neutral. We provide more information on the sampling procedure and on this stratified sample in Section \ref{appendix:initial_sample}.


% As our constraint is that we wish to annotate a limited amount of data for hate speech detection, we take some precautions to maximize the information found in our training dataset. For instance, if we were to sample randomly our collected tweets, we would face a strong imbalance in our data, as this strategy would yield very few positives, i.e. hateful tweets, and this scarcity would be even more marked for certain targeted communities. 

% To overcome this issue, we attempt oversampling tweets which contain hate, and which target our communities of interest such that the resulting. To do so, we perform a keyword-based stratified sampling. 
% This yields a subset of tweets where at least one community often subject to hate speech is mentioned, referred to as the \textit{community set} thereafter.
% \footnote{For more details about this set, please refer to \cref{app:community-set}} In this set, the prevalence of hate speech is presumably higher, reducing the class imbalance and simplifying its detection. 

% We further annotate this set as detailed in \cref{app:annotation-guidelines}.
%As previously stated\manu{this must be stated earlier in intro and/or related work}, the extreme imbalance in our classification task makes random sampling ineffective and prohibitively expensive. With the aim to build high-performing classifiers at a reasonable cost, we build and annotate a stratified sample of tweets from the community sampling set $C_s$. We use three different sampling strategies to build this stratified sample. First, for each possible combination of community name and hate word, we sample up to 4 tweets that both contain the respective hate word and match with the respective community regular expression. Second, for each combined word W, we randomly sample 50 tweets containing W. Finally, for each community, we draw 50 random tweets matching with the community regular expression, in order to avoid having a classifier that associates the community name with hate speech.
% This yields a stratified sample of 1,607 tweets annotated as either hateful, offensive or neutral, including 528 hateful tweets with annotated targets. We provide more information on the sampling procedure and on the initial stratified sample in Section \ref{app:stratified-sample}. 


%\paragraph{Hate words and targeted communities}
% To this end, we next present the annotation strategy suited for active learning used to train our models. 
% We first draw a stratified sample of tweets that can then be annotated and used for supervised learning\karim{what task ?}.
% \Karim{It is unclear what is stratified, the paragraph title mentions both hate detection and target detection. We could be more specific ?} To this end, w
% Specifically, we generate lists of seed words that often appear in hate speech in the Nigerian context: on the one hand, words which are associated with hate, and on the other, words which are associated with each of our targeted communities of interest. % First, we define a list of seed words that often appear in hate speech in the Nigerian context. 
%Specifically, our list contains 3 categories of words: Nigerian-specific derogatory words, names of communities often targeted by hate speech in Nigeria and words combining a derogatory word and a community name (e.g. ``fulanimal''). 
% We provide the full list of hate, community and combined words and the community regular expressions in Section \ref{appendix:word_lists}. \Manu{To do: add frequency, regex}
% \Karim{This portion is a bit long and contains some details that could go in the appendix. Would make it half a column}

% On the other, we create a dictionary of words associated with selected communities for target inference, in order to generate a community set relying on keyword and regular expressions matching, to cover the various ways these communities are talked about. In doing so, we chose to focus on the 12 most frequently mentioned communities, as this subset covers a large share of the Nigerian population. \karim{We need figures to support this claim: do we have stats?}
% We are aware that our matching doesn't capture all tweets mentioning a given community. However, these community sets are only the starting point for our active learning approach, detailed subsequently. 

% \Karim{As far as I understand we also annotated tweets in a random sample, we need to mention this and eventually give names to the sets in bold e.g. "community set" for AL training and "random test set" for evaluation purposes} 
% Additionally, we manually annotated a random sample for evaluation, independently from the automatic matching for community sets.

\Karim{The below is still unclear to me : do we use Fs apart from AL ? If it's only used for active learning I'd put it in the appendix along with AL details.}
Second, we aim to build a detection model that is robust to real-world conditions of extreme class imbalance. For this purpose, we draw a random sample of 200 million tweets out of the full Twitter dataset. As previously, we then split it randomly into two equally sized sets $F_s$ and $F_e$ that we use respectively for sampling and evaluation. 

\paragraph{Target inference dataset}
Further, we annotate positives, that is hateful tweets, with their target. As this is a multilabel problem, each tweet can be assigned several positives among our communities of interest. Specifically, we annotate positives from the stratified sample with X binary labels. \karim{Edit this and make sure it is clear which set is used for this problem}



% \paragraph{Data annotation}
% \Karim{Instead of having a "hate words and targeted communities" AND "Data annotation" paragraph, I would have a "Hate speech" paragraph and a "Targeted community" paragraph, where both the auxiliary data (words, etc) and annotation processes are described. I'd also present the stratified sample in the first one, and split evaluation between each}
% \Manu{The stratification is based on hate words + community words so it concerns both and cannot only appear in an independent hate speech paragraph}
% The subsequent tweet annotation of tweets is two-fold. 


% While we chose a prescriptive approach \cite{rottger2021two} to allow for policy relevance in light of content moderation, we account for cultural differences \cite{maronikolakis2022-listening} by engaging a diversity of annotators who were guided by a field coordinator with regional expertise. \Fixme{[More details on this pool of annotators]}

% \Todo{Include definition, references for guidelines. All tweets labeled at least twice and three times in case of disagreement (in case of disagreement with three labels, drop; if unsure label + ibrahims label, ibrahims has priority).} 

% \manu{Potentially make a table with examples of hate against each community}

% \paragraph{Sampling and evaluation random samples}

% While most hate speech classifiers are evaluated on random samples of curated datasets where the class imbalance is limited, we aim to evaluate our classifier in real-world settings of extreme imbalance. Specifically, we aim to evaluate our classifier (i) in the subset of all tweets containing at least one community name on the one hand, and (ii) on all tweets on the other hand.

% First, using the community regular expressions defined earlier and detailed in Section \ref{appendix:word_lists}, we select the subset of tweets that match with at least one community regular expression, totaling 42 million tweets and referred to as the \textit{community set} thereafter. We then randomly split this community set into two equally-sized sets $C_s$ and $C_e$ that we use respectively for sampling and evaluation. 

% Second, we draw a random sample of 200 million tweets out of the full Twitter dataset. As previously, we then split it randomly into two equally sized sets $F_s$ and $F_e$ that we use respectively for sampling and evaluation.
% \Fixme{Say a word on the fact that most classifiers are evaluated on curated/small datasets, not clear how they perform in real-settings of extreme imbalance}



% \Karim{Would put both "Data annotation" and "Initialization sample" in the appendix, or move to the previous section}
% \Manu{@Karim: with the new structure, I think it's important to keep them }

\subsection{Models and Baselines}\label{models}
% \subsubsection{Classification tasks}
% \paragraph{Hate speech detection}
% Following our data annotation task, we classify our collected tweets into three mutually-exclusive tweet categories: ``neutral'', ``offensive'' and ``hateful''. We give more details about the definition of such classes in Section \ref{appendix:labeling_guidelines} of the Appendix. \manu{This may be repetitive after detailing the annotation guidelines in the previous subsection?}
% % To compare our models, we report their \karim{Add metric}...

 
% \paragraph{Target inference}
% Once a hateful or offensive tweet is detected, our goal is to detect the target of hate. We frame this as a multi-label classification problem as multiple communities can be targeted in the same tweet. In particular, we detect which of the 12 classes described in \cref{hate_target_lists} are targeted. 
% Here, we rely on macro-F1 score for model comparison. \karim{add subtleties and challenges later : imbalance...}

% \subsubsection{Models}

\paragraph{Supervised learning}
For SL, we use \textbf{Conversational BERT} \cite{burtsev-etal-2018-deeppavlov}, a vanilla BERT base model further pre-trained on English social media data. We benchmarked several BERT-based models, including models trained on African languages \cite{ogueji-etal-2021-small, alabi-etal-2022-adapting}, and found that Conversational BERT had the best performance on our tasks. 

% \Fixme{[add literature on adapting pre-training language models to African languages: AfriBERTa \cite{ogueji-etal-2021-small}, AfroXLM-R \cite{alabi-etal-2022-adapting}]}

% \Todo{Details on fine-tuning}


\paragraph{Off-the-shelf models}
We mainly emply two off-the-shelf models. First, we use ChatGPT/GPT-3.5\footnote{\url{https://openai.com/blog/chatgpt}} which is based on the GPT-3 model \cite{brown2020language} and was further trained with Reinforcement Learning with Human Feedback (RLHF). We use this model in both a zero-shot learning ($GPT_{3.5}^{ZSL}$) and a few-shot learning ($GPT_{3.5}^{FSL}$) setting. We provide additional details on the prompts used for prediction in Section \ref{llms_prompts}. We also use Perspective API \cite{lees2022new}, a widely-deployed toxic language detection system based on BERT-based multilingual classifiers. Because of how the model was built, we can only use it for binary HSD and not for 3-class HSD nor TI.

% \Manu{[Perspective API is only used for binary hate speech detection, doesn't allow for multiclass hate speech detection nor target inference]}
% \Karim{cite paper for perspective api release and describe}.

\paragraph{Active Learning}
We use pool-based AL \cite{settles2009active} in batch mode. Specifically, we use \textbf{Certainty Sampling} \cite{attenberg2010unified} which aims to maximize precision by querying instances for which the model is most confident of their positivity. We choose this approach as we primarily care about model precision and because past work shows that it performs equally compared to other AL approaches under extreme imbalance \cite{tonneau2022multilingual}.
% ChatGPT has been shown to perform well in a zero-short learning setting, and on a variety of NLP tasks \cite{yuan-etal-2023-zero, jahan-etal-2023-evaluation, heck-etal-2023-chatgpt}. This makes it appealing as deploying such method does not require any human annotation efforts -- the extensive coverage of the model's training data suffices to handle with a variety of downstream tasks and domains. By designing simple prompts, this tool can be deployed in our scenario on both of our tasks, thanks to its versatility. 

% \Karim{Describe prompts used for ChatGPT. Mention it is used for hate speech detection and target inference};
% Perspective API in turn is a tool which is designed to reduce toxicity online, as it can detect hateful or abusive content from text. As such, it can be employed to automatically tag messages by whether they contain abuse or harassment. 


% \paragraph{Model evaluation}
% \Todo{Precision overall and by community}
% \Karim{Same, remove this one and put details in "tasks" ?}

% \subsection{Classification tasks}
% \paragraph{Hate speech detection}
% For our hate speech detection task, we classify our collected tweets into three mutually-exclusive tweet categories: ``neutral'', ``offensive'' and ``hateful''. We give more details about the definition of such classes in App \karim{add appendix}. 
% To compare our models, we report their \karim{Add metric}...

 
% \paragraph{Target inference}
% Once a hateful or offensive tweet is detected, our goal is to detect the target of hate. We frame this as a multi-label classification problem as multiple communities can be targeted in the same tweet. In particular, we detect which of the 12 classes described in \cref{sec:data} are targeted. 
% Here, we rely on macro-F1 score for model comparison. \karim{add subtleties and challenges later : imbalance...}

% \subsection{Active Learning}
% % Active learning (AL) has been successfully deployed in a variety of settings to reach robust performance on NLP tasks with limited
% % labeling efforts \cite{zhang-2019, griesshaber-etal-2020-fine, shelmanov-etal-2021-active, liu-2022, schroder-etal-2022-revisiting}. Another advantage of AL is that it also works for (extremely) imbalanced problems on social media \cite{palakodety2020voice, tonneau2022multilingual} the sampling strategy corrects these disparities. Further, this approach has been shown to successfully detect toxic content \cite{kirk-etal-2022-data}. 
% % In this work, we employ this strategy to iteratively help the model discriminate examples based on its likelihood on a limited number of examples, as our goal is to rely on limited labelling efforts. 


% Next, we investigate whether pool-based AL \cite{settles2009active} in batch mode allows to improve the classification performance of supervised learning at a limited cost. We specifically use \textbf{Certainty Sampling} \cite{attenberg2010unified} which aims to maximize precision by querying instances for which the model is most confident of their positivity. We choose this approach as we primarily care about model precision and because past work shows that it performs equally compared to other AL approaches under extreme imbalance \cite{tonneau2022multilingual}




% We do so on our hate speech detection task. At each AL iteration, we then perform a \textbf{certainty sampling} strategy in which we draw a fixed number of examples from five different buckets defined by the output likelihood of the model. 
% \Manu{we choose certainty sampling because we care mostly about precision and because past work shows that it performs equally compared to other AL approaches under extreme imbalance \cite{tonneau2022multilingual}} 

% Our initial goal is to maximize the performance of the classifier on the community set where the class imbalance is not as extreme as in the full set of tweets. For this purpose, we start performing AL on the community sampling set $C_s$ and evaluate the model on the community evaluation set $C_e$. Once the performance is satisfactory on the community set, we aim to maximize the performance of the classifier on the full set of tweets. We therefore continue performing AL but this time on the full sampling set $F_s$ and evaluate the model on the full evaluation set $F_e$. We run a total of 25 iterations, with each iteration sampling 100 tweets and of which 10 are run on $C_s$ and 15 on $F_s$.  

% Our final annotated dataset after AL contains 4,012 tweets annotated as either hateful, offensive or neutral.


% \Manu{We need a discussion somewhere on the target annotation. We basically label for targets all tweets characterized as hateful in the stratified sample, the AL samples and the evaluation samples. }

% Specifically, we initialize our model using a sample that is stratified by \textbf{community sets}, as described earlier. At each AL iteration, we then perform a \textbf{certainty sampling} strategy in which we draw a fixed number of examples from five different buckets defined by the output likelihood of the model. 
% \Karim{Add details here or in appendix, for number of examples, bucket intervals, number of iterations, etc.}
% \karim{Do we employ active learning for target inference as well ?}\manu{no, we don't. that's what we discussed doing on the fairness side but ended up dropping}

% \paragraph{Descriptive statistics}
% \Manu{Question of annotator agreement on labels to discuss somewhere}

\subsection{Evaluation}

\Fixme{Evaluation in the wild: average precision, recall is hard to compute}

\Fixme{Target inference: Here, we rely on macro-F1 score for model comparison. }
\karim{add subtleties and challenges later : imbalance...}

==> tables/krippendorff.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
                                  & $\alpha$ \\ \hline
Stratified + active learning sets &   0.68    \\ \hline
Top-scored evaluation set &   0.43    \\ \hline
Random set                        &   0.4                 \\ \hline
Full dataset                      &                    \\ \hline
\end{tabular}%
}
\caption{Inter-annotator agreement in terms of Krippendorff $\alpha$ across datasets}
\label{tab:krippendorff}
\end{table}
